A Bayesian Hierarchical Score for Structure Learning from Related Data Sets

Score functions for learning the structure of Bayesian networks in the literature assume that data are a homogeneous set of observations; whereas it is often the case that they comprise different related, but not homogeneous, data sets collected in different ways. In this paper we propose a new Bayesian Dirichlet score, which we call Bayesian Hierarchical Dirichlet (BHD). The proposed score is based on a hierarchical model that pools information across data sets to learn a single encompassing network structure, while taking into account the differences in their probabilistic structures. We derive a closed-form expression for BHD using a variational approximation of the marginal likelihood, we study the associated computational cost and we evaluate its performance using simulated data. We find that, when data comprise multiple related data sets, BHD outperforms the Bayesian Dirichlet equivalent uniform (BDeu) score in terms of reconstruction accuracy as measured by the Structural Hamming distance, and that it is as accurate as BDeu when data are homogeneous. This improvement is particularly clear when either the number of variables in the network or the number of observations is large. Moreover, the estimated networks are sparser and therefore more interpretable than those obtained with BDeu thanks to a lower number of false positive arcs.

==> model/model_BN.tex <==
\begin{tikzpicture}[x=1.7cm,y=1.8cm]

  % Nodes

  \node[obs]                   (X)      {$X_i| \mathrm{Pa}_i=\mathrm{pa}$} ; %
 \node[latent, left=of X]    (theta)  {$\boldsymbol{\theta}_{X_i| \mathrm{pa}}$}; %
  \node[latent, left=of theta] (alpha) {$\boldsymbol{\alpha}$};
  \node[const, left=of alpha] (alpha0) {$\boldsymbol{\alpha}_0$};
 
 
 
  % Factors
  \factor[left=of X]     {X-f}     {Cat.} {} {} ; %
   \factor[left=of theta] {theta-f} {Dir.} {} {} ; %
 \factor[left=of alpha] {alpha-f} {Dir.} {} {} ; %
 \node[const, below=of alpha-f, yshift=+1cm] (s) {$s$};

 
   \factoredge {theta}    {X-f}     {X} ; %
  \factoredge {alpha}    {theta-f}     {theta} ; %
  \factoredge {alpha0}    {alpha-f}     {alpha} ; %
  \factoredge    {alpha-f} {s}  {alpha-f}; %
  
  \plate {plate1} { %
    (X)
    (theta)
  } {$\forall \mathrm{pa} \in  \mathcal{P}_i$}; %
  \plate {plate2} { %
    (plate1)
    (alpha)
  } {$\forall i \in  \{1, \ldots, I\}$}; %
 
\end{tikzpicture}


==> model/model_hier.tex <==
\begin{tikzpicture}[x=1.7cm,y=1.8cm]

  % Nodes

  \node[obs]                   (X)      {$X| Y=y$} ; %
  \node[latent, left=of X]    (theta)  {$\boldsymbol{\theta}_{X|y}$}; %
  \node[latent, left=of theta] (alpha) {$\boldsymbol{\alpha}$};
  \node[const, left=of alpha] (alpha0) {$\boldsymbol{\alpha}_0$};
 

  % Factors
  \factor[left=of X]     {X-f}     {Cat.} {} {} ; %
  \factor[left=of theta] {theta-f} {Dir.} {} {} ; %
 \factor[left=of alpha] {alpha-f} {Dir.} {} {} ; %
 \node[const, below=of alpha-f, yshift=+1cm] (s) {$s$};

    \factoredge {theta}    {X-f}     {X} ; %
  \factoredge {alpha}    {theta-f}     {theta} ; %
  \factoredge {alpha0}    {alpha-f}     {alpha} ; %
  \factoredge    {alpha-f} {s}  {alpha-f}; %
  

  
  \plate {plate1} { %
    (X)
    (theta)
  } {$\forall y \in  \mathcal{Y}$}; %
 
\end{tikzpicture}


==> model/model_hier_VI.tex <==
\begin{tikzpicture}[x=1.7cm,y=1.8cm]

  % Nodes

  \node[obs]                   (X)      {$\XPi=j$} ; %
  \node[latent, left=of X]    (theta)  {$\tXi$}; %
   \node[latent, left=of theta]    (nu)  {$\boldsymbol{\nu}_{j}$}; %
 \node[latent, left=of nu] (alpha) {$\boldsymbol{\alpha}$};
  \node[latent, left=of alpha] (alpha0) {$\tau \boldsymbol{\kappa}$};

   \node[obs, above=of X]                   (X_h)      {$\XPi=j$} ; %
  \node[latent, left=of X_h]    (theta_h)  {$\tXi$}; %
  \node[latent, left=of theta_h, xshift=-2.4cm] (alpha_h) {$\boldsymbol{\alpha}$};
  \node[const, left=of alpha_h] (alpha0_h) {$\boldsymbol{\alpha}_0$};
 

 
  % Factors
  \factor[left=of X]     {X-f}     {Cat.} {} {} ; %
 \factor[left=of theta] {theta-f} {Dir.} {} {} ; %
 \factor[left=of alpha] {alpha-f} {Dir.} {} {} ; %
 \node[const, below=of alpha-f, yshift=+1cm] (s) {$s$};
  \factor[left=of X_h]     {X-f_h}     {Cat.} {} {} ; %
  \factor[left=of theta_h, xshift=-1.4cm] {theta-f_h} {Dir.} {} {} ; %
 \factor[left=of alpha_h] {alpha-f_h} {Dir.} {} {} ; %
 \node[const, below=of alpha-f_h, yshift=+1cm] (s_h) {$s$};

 
   \factoredge {theta}    {X-f}     {X} ; %
  \factoredge {nu}    {theta-f}     {theta} ; %
  \factoredge {alpha0}    {alpha-f}     {alpha} ; %
  \factoredge    {alpha-f} {s}  {alpha-f}; %
     \factoredge {theta_h}    {X-f_h}     {X_h} ; %
  \factoredge {alpha_h}    {theta-f_h}     {theta_h} ; %
  \factoredge {alpha0_h}    {alpha-f_h}     {alpha_h} ; %
  \factoredge    {alpha-f_h} {s_h}  {alpha-f_h}; %

\plate {plate} { %
    (X_h)
    (theta_h)
  } {$\forall j \in  1, \ldots, |\PXi|$}; %
  \plate {plate1} { %
    (X)%
    (theta)
    (nu)
  } {$\forall j \in 1, \ldots, |\PXi| $}; %
 
\end{tikzpicture}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

